Sea-Net: A Small and Inherently Interpretable Neural Network for Time Series Classification

Traditional time-series classification methods often operate as black boxes, providing a class prediction without indicating which time point or time interval within the series led to that prediction. To improve temporal interpretability, MILLET (Multiple Instance Learning with Temporal Explanation), which combines an InceptionTime encoder with Conjunctive Pooling, provides both classification and temporal explanations. However, MILLET contains approximately 424 K parameters, making it unsuitable for deployment on resource-constrained micro-controllers, and it achieves an overall time-series accuracy of 0.888 and an explanation score of 0.681 NDCG@n. We therefore propose SEA-Net, a lightweight architecture using small multi-scale depthwise-separable convolutional TSC encoders and improved Multiple Instance Learning (MIL) pooling heads. Our SEA-Net bottleneck encoder with Top-k pooling achieves 0.931 accuracy and 0.765 NDCG@n with only 41 K parameters. Another variant, using a gated encoder with Top-k pooling, achieves 0.955 accuracy and 0.750 NDCG@n with 62 K parameters. These results demonstrate that lightweight architectures can maintain strong classification performance and temporal explanations while substantially reducing model size. The proposed variants address specific limitations of the pooling strategy used by MILLET, providing a practical direction for interpretable time-series classification on resource-constrained edge devices.

==> figures/fig_block_tikz.tex <==
% !TEX root = ../internsip_ubaid.tex
% =====================================================================
% fig_block_tikz.tex -- the zoom-in on ONE multi-scale separable block.
%
% Drawn in TikZ instead of an image file, so it stays sharp and so the
% numbers on it can never drift away from the text.
% Source of truth: seanet/features.py, class MultiScaleSepBlock.forward()
%
% This file is pulled in by sections/05_architecture.tex with \input, and
% that \input sits inside \ifshowblockfig ... \fi. So it is OPTIONAL:
% set \showblockfigfalse in preamble.tex and the whole thing disappears
% without touching anything else.
%
% Two panels:
%   (a) the data path through one unit, the "x2", and the residual add
%   (b) the receptive field: same 5 taps, dilation 1 against dilation 16
% =====================================================================

% ---- panel (a): the data path ---------------------------------------
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}[
  font=\small,
  >={Stealth[length=2mm]},
  % a convolution branch: the three of them differ only in kernel size
  conv/.style   = {draw=orange!65!black, fill=orange!18, rounded corners=2pt,
                   minimum height=8mm, inner xsep=4pt, align=center},
  % the cheap "mix and clean up" steps after the sum
  stage/.style   = {draw=black!55, fill=black!7, rounded corners=2pt,
                   minimum height=8mm, minimum width=11mm, align=center},
  % the tensors going in and out
  tensor/.style = {draw=black!45, fill=black!3, rounded corners=2pt,
                   minimum height=11mm, minimum width=13mm, align=center},
  op/.style     = {draw=black!65, circle, inner sep=1pt, minimum size=5.5mm},
]

% --- input ------------------------------------------------------------
\node[tensor] (h) at (0,0) {$\mathbf{h}$\\[1pt]\scriptsize$(B,d,\nsteps)$};

% --- the three depthwise convolutions, one per kernel size ------------
% drawn with increasing width, so "wider box = looks further in time"
\node[conv, minimum width=20mm] (k5)  at (3.7, 1.7) {depthwise $k{=}5$\\[-1pt]\scriptsize dilation $\delta$, groups $=d$};
\node[conv, minimum width=26mm] (k11) at (3.7, 0.0) {depthwise $k{=}11$\\[-1pt]\scriptsize dilation $\delta$, groups $=d$};
\node[conv, minimum width=32mm] (k23) at (3.7,-1.7) {depthwise $k{=}23$\\[-1pt]\scriptsize dilation $\delta$, groups $=d$};

\draw[->] (h.east) -- ++(0.4,0) |- (k5.west);
\draw[->] (h.east) -- ++(0.4,0) |- (k11.west);
\draw[->] (h.east) -- ++(0.4,0) |- (k23.west);

% --- they are simply added together -----------------------------------
\node[op] (sum) at (6.9,0) {$+$};
\draw[->] (k5.east)  -| (sum.north);
\draw[->] (k11.east) -- (sum.west);
\draw[->] (k23.east) -| (sum.south);

% --- mix the channels, normalise, activate, regularise ----------------
\node[stage] (pw)   at ( 8.9,0) {$1{\times}1$\\[-1pt]pointwise};
\node[stage] (bn)   at (10.7,0) {BatchNorm};
\node[stage] (relu) at (12.4,0) {ReLU};
\node[stage] (drop) at (14.0,0) {Dropout};

\draw[->] (sum.east)  -- (pw.west);
\draw[->] (pw.east)   -- (bn.west);
\draw[->] (bn.east)   -- (relu.west);
\draw[->] (relu.east) -- (drop.west);

% --- the residual add that closes the block ---------------------------
\node[op] (add) at (16.0,0) {$+$};
\node[stage, minimum width=9mm] (outrelu) at (17.6,0) {ReLU};
\node[tensor] (out) at (19.6,0) {output\\[1pt]\scriptsize$(B,d,\nsteps)$};

\draw[->] (drop.east)     -- (add.west);
\draw[->] (add.east)      -- (outrelu.west);
\draw[->] (outrelu.east) -- (out.west);

% the skip connection: the BLOCK's own input, carried over the top
\draw[->, thick, black!60] (h.north) |- (0,3.0) -| node[pos=0.25, above, black!60]
      {\small skip connection: the block's own input $\mathbf{h}$} (add.north);

% --- the dashed box marking what gets repeated twice ------------------
\begin{scope}[on background layer]
  \node[draw=black!55, dashed, rounded corners=3pt, inner sep=7pt,
        fit=(k5)(k23)(drop)] (unitbox) {};
\end{scope}
% the label sits UNDER the dashed box, where nothing else is drawn
\node[anchor=north west, black!70] at ($(unitbox.south west)+(2pt,-1pt)$)
      {\small \textbf{one unit} -- run twice, back to back ($\times 2$)};

\end{tikzpicture}}

\vspace{5pt}

% ---- panel (b): the receptive field ---------------------------------
\resizebox{0.92\linewidth}{!}{%
\begin{tikzpicture}[x=0.185cm, y=1cm, font=\small, >={Stealth[length=1.6mm]}]

% ---- top row: dilation 1 --------------------------------------------
% 65 input positions; the k=5 filter takes 5 neighbouring points
\foreach \i in {0,...,64} { \fill[black!22] (\i,0) circle (0.5mm); }
\foreach \i in {30,31,32,33,34} {
  \draw[orange!65!black, thin] (\i,0) -- (32,0.85);
  \fill[orange!75!black] (\i,0) circle (0.9mm);
}
\fill[black!80] (32,0.85) circle (1.1mm);
\node[anchor=west, black!80] at (34,0.85) {\ one output value};
\node[anchor=east] at (-1.5,0) {$\delta = 1$\ };
\node[anchor=north, black!60] at (32,-0.30) {\small sees 5 time steps in a row};

% ---- bottom row: dilation 16 ----------------------------------------
\begin{scope}[yshift=-2.1cm]
\foreach \i in {0,...,64} { \fill[black!22] (\i,0) circle (0.5mm); }
\foreach \i in {0,16,32,48,64} {
  \draw[orange!65!black, thin] (\i,0) -- (32,0.85);
  \fill[orange!75!black] (\i,0) circle (0.9mm);
}
\fill[black!80] (32,0.85) circle (1.1mm);
\node[anchor=west, black!80] at (34,0.85) {\ one output value};
\node[anchor=east] at (-1.5,0) {$\delta = 16$\ };
\node[anchor=north, black!60] at (32,-0.30)
     {\small the same 5 taps, now spread over 65 time steps};
% the reach, drawn as a measured bar
\draw[<->, black!55] (0,-0.95) -- node[below, black!55, font=\small] {receptive field} (64,-0.95);
\end{scope}

\end{tikzpicture}}


==> tables/01_main/tab03_cost/tab03_cost_ver1.tex <==
% tab03_cost - corrected layout (Series/s, Peak GPU mem and Train time removed; short column names; all data columns centred).
\begin{table}[tbp]
\caption{Cost on the WebTraffic input (length 1{,}008, 10 classes), one GPU, batch 32. \emph{Params}$\times$ and \emph{FLOPs}$\times$ are size and compute relative to the re-trained MILLET baseline; column definitions in Appendix~\ref{app:metrics}; lower is better throughout.}
\label{tab:cost}
\begin{center}
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.15}
\ifdefined\seatablebox\else\newsavebox\seatablebox\fi
\sbox\seatablebox{\begin{tabular}{lcccccc}
\toprule
\textbf{Model} & \textbf{Params} & \textbf{Size} & \textbf{FLOPs} & \textbf{Latency} & \textbf{Params}$\times$ & \textbf{FLOPs}$\times$ \\
\midrule
\multicolumn{7}{l}{\emph{SEA-Net (ours)}} \\
bottleneck + Top-$k$ conj. & \textbf{41{,}324} & \textbf{1.43} & \textbf{76.7} & 0.131 & 0.10$\times$ & 0.09$\times$ \\
bottleneck + Top-$k$ conj. ($\lambda_{\text{focus}}=0$) & \textbf{41{,}324} & \textbf{1.43} & \textbf{76.7} & 0.130 & 0.10$\times$ & 0.09$\times$ \\
input-gated + Top-$k$ conj. & 58{,}092 & 1.49 & 110.6 & 0.130 & 0.14$\times$ & 0.13$\times$ \\
gated (mean) + Top-$k$ conj. & 61{,}740 & 1.50 & 109.7 & 0.128 & 0.15$\times$ & 0.13$\times$ \\
spike/trend + Top-$k$ conj. & 67{,}020 & 1.53 & 120.1 & 0.132 & 0.16$\times$ & 0.14$\times$ \\
bottleneck + Top-$k$ conj., 2026-09 re-run & \textbf{41{,}324} & \textbf{1.43} & \textbf{76.7} & 0.131 & 0.10$\times$ & 0.09$\times$ \\
\midrule
\multicolumn{7}{l}{\emph{Baselines}} \\
MILLET (InceptionTime + conjunctive), our recipe & 423{,}707 & 4.11 & 847.6 & 0.203 & 1.00$\times$ & 1.00$\times$ \\
MILLET, their recipe (1500 epochs, no early stopping) & 423{,}707 & 4.11 & 847.6 & 0.202 & 1.00$\times$ & 1.00$\times$ \\
ResNet + conjunctive & 506{,}331 & 4.42 & 1013.2 & 0.139 & 1.20$\times$ & 1.20$\times$ \\
FCN + conjunctive & 267{,}035 & 3.47 & 535.2 & \textbf{0.068} & 0.63$\times$ & 0.63$\times$ \\
\bottomrule
\end{tabular}}
\ifdim\wd\seatablebox>\linewidth
  \resizebox{\linewidth}{!}{\usebox\seatablebox}
\else
  \usebox\seatablebox
\fi
\end{center}
\end{table}


==> tables/leaderboard.tex <==
% GENERATED by scripts/make_leaderboard_tex.py from
% results/SEA_NET/leaderboard.csv -- do not edit by hand.
{\scriptsize
\setlength{\tabcolsep}{3pt}
\begin{longtable}{rlllcccrr}
\caption{All 72 encoder--head combinations, ordered by \webtraffic{} accuracy. A dash in the
\ucr{} column means the combination was tested on \webtraffic{} only. Pooling heads marked
$^{*}$ are \millet{}'s own, used unchanged.}
\label{tab:app_leaderboard} \\
\toprule
\# & \textbf{Configuration} & \textbf{Encoder} & \textbf{Head} &
Acc. & AOPCR & \ndcg{} & \ucr{}-85 & Params \\
\midrule
\endfirsthead
\multicolumn{9}{l}{\emph{\Cref{tab:app_leaderboard} continued from the previous page.}} \\
\toprule
\# & \textbf{Configuration} & \textbf{Encoder} & \textbf{Head} &
Acc. & AOPCR & \ndcg{} & \ucr{}-85 & Params \\
\midrule
\endhead
\midrule
\multicolumn{9}{r}{\emph{continued on the next page}} \\
\endfoot
\bottomrule
\endlastfoot
1 & \texttt{seanet\_gated\_mean\_topk} & gated & Top-$k$ & 0.955 & 2.23 & 0.750 & 0.8083 & 61{,}740 \\
2 & \texttt{seanet\_conjunctive} & plain & conjunctive* & 0.954 & 1.50 & 0.698 & 0.8238 & 269{,}083 \\
3 & \texttt{seanet\_gated\_max\_topk} & gated & Top-$k$ & 0.952 & 2.27 & 0.719 & 0.8108 & 61{,}740 \\
4 & \texttt{seanet\_topk\_nofocus} & bottleneck & Top-$k$ & 0.950 & 2.30 & 0.765 & --- & 41{,}324 \\
5 & \texttt{seanet\_spiketrend\_topk} & spike/trend & Top-$k$ & 0.950 & 2.32 & 0.756 & 0.8089 & 67{,}020 \\
6 & \texttt{seanet\_inputgate\_mschan} & ms-channels & Top-$k$ & 0.948 & 2.32 & 0.757 & --- & 69{,}768 \\
7 & \texttt{seanet\_gated\_mschan} & ms-channels & Top-$k$ & 0.948 & 2.22 & 0.717 & --- & 67{,}592 \\
8 & \texttt{seanet\_bottleneck\_topk} & bottleneck & Top-$k$ & 0.947 & 2.62 & 0.772 & 0.8097 & 41{,}324 \\
9 & \texttt{seanet\_recon\_adaptive} & recon & adaptive & 0.946 & 2.60 & 0.768 & 0.8140 & 62{,}935 \\
10 & \texttt{seanet\_inputgate\_topk} & input-gated & Top-$k$ & 0.946 & 2.80 & 0.748 & 0.8131 & 58{,}092 \\
11 & \texttt{seanet\_classwise} & plain & class-wise & 0.946 & 1.72 & 0.686 & 0.8292 & 269{,}164 \\
12 & \texttt{seanet\_gated\_max} & gated & class-wise & 0.944 & 1.89 & 0.592 & 0.8237 & 61{,}740 \\
13 & \texttt{seanet\_gated\_last\_topk} & gated & Top-$k$ & 0.942 & 2.31 & 0.748 & 0.8015 & 61{,}740 \\
14 & \texttt{seanet} & plain & additive* & 0.942 & 1.58 & 0.729 & 0.8298 & 269{,}083 \\
15 & \texttt{seanet\_gated\_last} & gated & class-wise & 0.942 & 2.52 & 0.742 & 0.7888 & 61{,}740 \\
16 & \texttt{seanet\_recon\_topk} & recon & Top-$k$ & 0.940 & 2.51 & 0.698 & 0.8063 & 62{,}925 \\
17 & \texttt{seanet\_topk\_k025} & bottleneck & Top-$k$ & 0.940 & 2.65 & 0.733 & --- & 41{,}324 \\
18 & \texttt{seanet\_bottleneck\_softmax} & bottleneck & softmax & 0.940 & 1.68 & 0.740 & 0.8106 & 41{,}325 \\
19 & \texttt{seanet\_gated\_last\_adaptive} & gated & adaptive & 0.938 & 2.39 & 0.793 & 0.8029 & 61{,}750 \\
20 & \texttt{seanet\_spiketrend\_adaptive} & spike/trend & adaptive & 0.934 & 1.91 & 0.747 & 0.8010 & 67{,}030 \\
21 & \texttt{seanet\_recon\_softmax} & recon & softmax & 0.932 & 1.64 & 0.723 & --- & 62{,}926 \\
22 & \texttt{seanet\_slim\_topk} & plain & Top-$k$ & 0.932 & 2.69 & 0.778 & 0.8093 & 57{,}580 \\
23 & \texttt{seanet\_bottleneck\_gatedattn} & bottleneck & gated-attn & 0.930 & 2.23 & 0.741 & 0.8146 & 41{,}844 \\
24 & \texttt{seanet\_spiketrend\_gatedattn} & spike/trend & gated-attn & 0.930 & 1.59 & 0.721 & 0.8039 & 67{,}540 \\
25 & \texttt{seanet\_gated} & gated & class-wise & 0.930 & 2.41 & 0.637 & 0.7900 & 61{,}740 \\
26 & \texttt{seanet\_slim\_adaptive} & plain & adaptive & 0.930 & 2.45 & 0.793 & --- & 57{,}590 \\
27 & \texttt{seanet\_bottleneck\_mschan} & ms-channels & Top-$k$ & 0.926 & 2.24 & 0.777 & --- & 47{,}176 \\
28 & \texttt{seanet\_bottleneck\_mschan\_lean} & ms-channels & Top-$k$ & 0.924 & 2.76 & 0.735 & --- & 43{,}576 \\
29 & \texttt{seanet\_gated\_last\_softmax} & gated & softmax & 0.920 & 1.99 & 0.738 & --- & 61{,}741 \\
30 & \texttt{millet\_paper} & InceptionTime & conjunctive* & 0.920 & 13.27 & 0.661 & 0.8434 & 423{,}707 \\
31 & \texttt{seanet\_acp} & plain & adaptive & 0.918 & 1.61 & 0.619 & 0.8134 & 269{,}174 \\
32 & \texttt{seanet\_gated\_last\_gatedattn} & gated & gated-attn & 0.918 & 1.35 & 0.757 & 0.8048 & 62{,}260 \\
33 & \texttt{seanet\_slim} & plain & class-wise & 0.916 & 2.48 & 0.719 & --- & 57{,}580 \\
34 & \texttt{seanet\_gated\_max\_softmax} & gated & softmax & 0.914 & 1.88 & 0.776 & --- & 61{,}741 \\
35 & \texttt{seanet\_inputgate} & input-gated & class-wise & 0.914 & 2.48 & 0.715 & --- & 58{,}092 \\
36 & \texttt{seanet\_gated\_mean\_softmax} & gated & softmax & 0.912 & 2.09 & 0.765 & --- & 61{,}741 \\
37 & \texttt{seanet\_recon} & recon & class-wise & 0.910 & 2.50 & 0.680 & --- & 62{,}925 \\
38 & \texttt{seanet\_topk\_k100} & bottleneck & Top-$k$ & 0.908 & 2.44 & 0.722 & --- & 41{,}324 \\
39 & \texttt{seanet\_gated\_max\_adaptive} & gated & adaptive & 0.906 & 2.07 & 0.729 & --- & 61{,}750 \\
40 & \texttt{seanet\_inputgate\_adaptive} & input-gated & adaptive & 0.905 & 2.65 & 0.732 & 0.8153 & 58{,}102 \\
41 & \texttt{seanet\_spiketrend} & spike/trend & class-wise & 0.904 & 2.15 & 0.699 & --- & 67{,}020 \\
42 & \texttt{seanet\_bottleneck} & bottleneck & class-wise & 0.902 & 2.57 & 0.733 & --- & 41{,}324 \\
43 & \texttt{seanet\_gated\_mean} & gated & class-wise & 0.902 & 2.49 & 0.714 & --- & 61{,}740 \\
44 & \texttt{seanet\_inputgate\_softmax} & input-gated & softmax & 0.894 & 1.64 & 0.696 & --- & 58{,}093 \\
45 & \texttt{seanet\_slim\_gatedattn} & plain & gated-attn & 0.894 & 2.30 & 0.714 & --- & 58{,}100 \\
46 & \texttt{seanet\_recon\_attnmax} & recon & attn-max & 0.892 & 2.32 & 0.725 & --- & 62{,}935 \\
47 & \texttt{seanet\_slim\_softmax} & plain & softmax & 0.890 & 1.83 & 0.705 & --- & 57{,}581 \\
48 & \texttt{seanet\_slim\_gatedattn} & gated & attention* & 0.888 & 2.40 & 0.710 & --- & 58{,}100 \\
49 & \texttt{seanet\_topk\_k005} & bottleneck & Top-$k$ & 0.888 & 2.29 & 0.715 & --- & 41{,}324 \\
50 & \texttt{millet} & InceptionTime & conjunctive* & 0.887 & 2.57 & 0.677 & 0.8274 & 423{,}707 \\
51 & \texttt{seanet\_gated\_max\_attnmax} & gated & attn-max & 0.886 & 1.12 & 0.575 & --- & 61{,}750 \\
52 & \texttt{seanet\_topk\_k050} & bottleneck & Top-$k$ & 0.882 & 3.11 & 0.732 & --- & 41{,}324 \\
53 & \texttt{seanet\_softmax} & plain & softmax & 0.880 & 1.02 & 0.605 & 0.8131 & 269{,}165 \\
54 & \texttt{seanet\_spiketrend\_softmax} & spike/trend & softmax & 0.878 & 1.43 & 0.665 & --- & 67{,}021 \\
55 & \texttt{seanet\_bottleneck\_adaptive} & bottleneck & adaptive & 0.868 & 1.97 & 0.680 & --- & 41{,}334 \\
56 & \texttt{seanet\_slim\_dualstream} & plain & dual-stream & 0.860 & 2.40 & 0.745 & --- & 58{,}101 \\
57 & \texttt{seanet\_gated\_mean\_adaptive} & gated & adaptive & 0.860 & 2.24 & 0.731 & --- & 61{,}750 \\
58 & \texttt{seanet\_inputgate\_attnmax} & input-gated & attn-max & 0.858 & 2.15 & 0.700 & --- & 58{,}102 \\
59 & \texttt{seanet\_spiketrend\_attnmax} & spike/trend & attn-max & 0.854 & 1.65 & 0.644 & --- & 67{,}030 \\
60 & \texttt{seanet\_gated\_last\_attnmax} & gated & attn-max & 0.854 & 1.78 & 0.668 & --- & 61{,}750 \\
61 & \texttt{seanet\_bottleneck\_shallow} & bottleneck & Top-$k$ & 0.846 & 2.82 & 0.624 & --- & 21{,}548 \\
62 & \texttt{seanet\_gated\_mean\_attnmax} & gated & attn-max & 0.832 & 1.67 & 0.704 & --- & 61{,}750 \\
63 & \texttt{seanet\_gated\_pyramid} & ms-pyramid & Top-$k$ & 0.832 & 0.98 & 0.591 & --- & 62{,}781 \\
64 & \texttt{seanet\_bottleneck\_dualstream} & bottleneck & dual-stream & 0.824 & 2.04 & 0.652 & --- & 41{,}845 \\
65 & \texttt{seanet\_bottleneck\_attnmax} & bottleneck & attn-max & 0.816 & 1.74 & 0.610 & --- & 41{,}334 \\
66 & \texttt{seanet\_bottleneck\_pyramid} & ms-pyramid & Top-$k$ & 0.786 & 1.03 & 0.569 & --- & 42{,}365 \\
67 & \texttt{resnet} & ResNet & conjunctive* & 0.772 & 2.95 & 0.554 & 0.8146 & 506{,}331 \\
68 & \texttt{fcn} & FCN & conjunctive* & 0.742 & 3.83 & 0.533 & 0.8141 & 267{,}035 \\
69 & \texttt{seanet\_gated\_last\_dualstream} & gated & dual-stream & 0.736 & 1.95 & 0.637 & --- & 62{,}261 \\
70 & \texttt{seanet\_slim\_attnmax} & plain & attn-max & 0.714 & 1.63 & 0.532 & --- & 57{,}590 \\
71 & \texttt{seanet\_bottleneck\_mschan\_pyramid} & ms-pyramid & Top-$k$ & 0.696 & 2.17 & 0.653 & --- & 28{,}441 \\
72 & \texttt{seanet\_spiketrend\_dualstream} & spike/trend & dual-stream & 0.556 & 1.64 & 0.510 & --- & 67{,}541 \\
\end{longtable}}

